Differentiation of Linear Optical Circuits

Linear optical circuits with single-photon sources offer a promising platform for quantum chemistry and machine learning. However, current applications are all based on support vector machines or gradient-free optimization methods. This paper develops classical and quantum algorithms for evaluating the analytic gradients of linear optical circuits with respect to their phase parameters. First, we set up a general framework by characterising the class of observables whose expectation values can be estimated efficiently by sampling from a passive linear optical circuit with finitely many photons. We then show how to compute the gradients of the expectation values of a special class of ``non-interacting'' observables arising in full-counting-statistics. Our differentiation algorithm uses the Halmos dilation and requires evaluating two circuits of twice the size, using one additional photon. Building on the methods of full-counting-statistics, we show how to recover the gradients of arbitrary observables from the gradient of a non-interacting characteristic function. Throughout the paper, we compare the performance of classical and quantum algorithms on the same estimation problems, analysing the sampling complexity of the algorithms and suggesting different cases for which quantum speed-ups could be obtained.

==> preamble/packages.tex <==
% https://mirror.ox.ac.uk/sites/ctan.org/macros/latex/contrib/pdfx/pdfx.pdf
%\usepackage[a-3b]{pdfx}
\usepackage[UKenglish]{babel}
\usepackage{fontenc}
\usepackage[utf8]{inputenc}

% Math Symbols
\usepackage{mathtools}
\usepackage{physics}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{mathdots}   % diagonal dots in other direction
\usepackage{mathrsfs}   % cursive font
\usepackage{bigints}    % for the use of bra and ket
\usepackage{xfrac}      % for \sfrac in powers
\usepackage{stmaryrd}   % doubled brackets
\SetSymbolFont{stmry}{bold}{U}{stmry}{m}{n}   % get rid of annoying warning from stmaryrd
\usepackage{extarrows} % \xLongrightarrow

% Theorem tools
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{thm-restate}

\usepackage{placeins}

\usepackage{bm}   % for \bm

\usepackage{blkarray}   % for row index of matrix

\usepackage{graphicx}
\graphicspath{figures}

%\usepackage{xcolor} % Already loaded by pdfx
\usepackage{tikzfig}
\usepackage{pgfplots} % For style=braceedge in TikZiT
\pgfplotsset{compat=newest, compat/show suggested version=false} % Some warning
\usepackage{tikz-cd}


% TikZiT style %
\input{preamble/zxw.tikzstyles}
\definecolor{zx_grey}{RGB}{211,211,211}
\definecolor{zx_red}{RGB}{232,165,165}
\definecolor{zx_green}{RGB}{216,248,216}
\definecolor{bluegray}{rgb}{0.4, 0.6, 0.8}

\usepackage{xtab}
\usepackage{tabu}
\usepackage{multicol}


% DarkMode :D
%\pagecolor[HTML]{282C34}
%\color[HTML]{979FAD}
%\hypersetup{linkcolor=cyan}

% "Basically, cleveref must be loaded last."
% https://anorien.csc.warwick.ac.uk/mirrors/CTAN/macros/latex/contrib/cleveref/cleveref.pdf
\usepackage[capitalise, noabbrev]{cleveref}


==> preamble/symbols.tex <==
% Number Rings %
\newcommand{\B}{\mathbb{B}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\renewcommand{\H}{\mathbb{H}}
\renewcommand{\O}{\mathbb{O}}
\ifdef{\C}
  {\renewcommand{\C}{\mathbb{C}}}
  {\newcommand{\C}{\mathbb{C}}}
% Shorter minus sign
\newcommand{\minu}{\texttt{-}}
\newcommand{\plus}{\texttt{+}}

% ZX interpretation
\newcommand{\tikzinterp}[1]{\left\llbracket\,#1\,\right\rrbracket}
\newcommand{\interp}[1]{\left\llbracket#1\right\rrbracket}
\newcommand{\ZX}{\mathsf{ZX}}

\newcommand{\bR}{\begin{color}{red}}
\newcommand{\bB}{\begin{color}{blue}}
\newcommand{\bM}{\begin{color}{magenta}}
\newcommand{\bC}{\begin{color}{cyan}}
\newcommand{\bW}{\begin{color}{white}}
\newcommand{\bBl}{\begin{color}{black}}
\newcommand{\bG}{\begin{color}{green}}
\newcommand{\bY}{\begin{color}{yellow}}
\newcommand{\e}{\end{color}}
\newcommand{\TODOb}[1]{\marginpar{\scriptsize\bR \textbf{TODO:} #1\e}}
\newcommand{\COMMb}[1]{\marginpar{\scriptsize\bM \textbf{COMM:} #1\e}}

\newcommand{\tikzrefsize}[1]{\scriptsize{#1}}
\newcommand{\axref}[1]{\tikzrefsize{\eqref{rule:#1}}}
\newcommand{\lemref}[1]{\tikzrefsize{\eqref{#1}}}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}
%======================================
\newtheorem{Th}{Theorem}[section]
\newtheorem{theorem}[Th]{Theorem}
\newtheorem{proposition}[Th]{Proposition} 
\newtheorem{lemma}[Th]{Lemma}
\newtheorem{corollary}[Th]{Corollary}
\newtheorem{definition}[Th]{Definition} 
\newtheorem{example}[Th]{Example}
\newtheorem{remark}[Th]{Remark}

%======================================
\newcommand{\rsnote}[1]{\marginpar{\scriptsize \bB \emph{RS:} #1 \e}}
\newcommand{\hwnote}[1]{\marginpar{\scriptsize \bR \emph{HW:} #1 \e}}

\newcommand{\zxw}[1]{\cite[#1]{poorCompletenessArbitraryFinite2023}}
\newcommand{\inftyfy}[1]{#1$\null_{\infty}$}

==> source/preamble/packages.tex <==
% https://mirror.ox.ac.uk/sites/ctan.org/macros/latex/contrib/pdfx/pdfx.pdf
%\usepackage[a-3b]{pdfx}
\usepackage[UKenglish]{babel}
\usepackage{fontenc}
\usepackage[utf8]{inputenc}

% Math Symbols
\usepackage{mathtools}
\usepackage{physics}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{mathdots}   % diagonal dots in other direction
\usepackage{mathrsfs}   % cursive font
\usepackage{bigints}    % for the use of bra and ket
\usepackage{xfrac}      % for \sfrac in powers
\usepackage{stmaryrd}   % doubled brackets
\SetSymbolFont{stmry}{bold}{U}{stmry}{m}{n}   % get rid of annoying warning from stmaryrd
\usepackage{extarrows} % \xLongrightarrow

% Theorem tools
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{thm-restate}

\usepackage{placeins}

\usepackage{bm}   % for \bm

\usepackage{blkarray}   % for row index of matrix

\usepackage{graphicx}
\graphicspath{figures}

%\usepackage{xcolor} % Already loaded by pdfx
\usepackage{tikzfig}
\usepackage{pgfplots} % For style=braceedge in TikZiT
\pgfplotsset{compat=newest, compat/show suggested version=false} % Some warning
\usepackage{tikz-cd}


% TikZiT style %
\input{preamble/zxw.tikzstyles}
\definecolor{zx_grey}{RGB}{211,211,211}
\definecolor{zx_red}{RGB}{232,165,165}
\definecolor{zx_green}{RGB}{216,248,216}
\definecolor{bluegray}{rgb}{0.4, 0.6, 0.8}

\usepackage{xtab}
\usepackage{tabu}
\usepackage{multicol}


% DarkMode :D
%\pagecolor[HTML]{282C34}
%\color[HTML]{979FAD}
%\hypersetup{linkcolor=cyan}

% "Basically, cleveref must be loaded last."
% https://anorien.csc.warwick.ac.uk/mirrors/CTAN/macros/latex/contrib/cleveref/cleveref.pdf
\usepackage[capitalise, noabbrev]{cleveref}


==> source/preamble/symbols.tex <==
% Number Rings %
\newcommand{\B}{\mathbb{B}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\renewcommand{\H}{\mathbb{H}}
\renewcommand{\O}{\mathbb{O}}
\ifdef{\C}
  {\renewcommand{\C}{\mathbb{C}}}
  {\newcommand{\C}{\mathbb{C}}}
% Shorter minus sign
\newcommand{\minu}{\texttt{-}}
\newcommand{\plus}{\texttt{+}}

% ZX interpretation
\newcommand{\tikzinterp}[1]{\left\llbracket\,#1\,\right\rrbracket}
\newcommand{\interp}[1]{\left\llbracket#1\right\rrbracket}
\newcommand{\ZX}{\mathsf{ZX}}

\newcommand{\bR}{\begin{color}{red}}
\newcommand{\bB}{\begin{color}{blue}}
\newcommand{\bM}{\begin{color}{magenta}}
\newcommand{\bC}{\begin{color}{cyan}}
\newcommand{\bW}{\begin{color}{white}}
\newcommand{\bBl}{\begin{color}{black}}
\newcommand{\bG}{\begin{color}{green}}
\newcommand{\bY}{\begin{color}{yellow}}
\newcommand{\e}{\end{color}}
\newcommand{\TODOb}[1]{\marginpar{\scriptsize\bR \textbf{TODO:} #1\e}}
\newcommand{\COMMb}[1]{\marginpar{\scriptsize\bM \textbf{COMM:} #1\e}}

\newcommand{\tikzrefsize}[1]{\scriptsize{#1}}
\newcommand{\axref}[1]{\tikzrefsize{\eqref{rule:#1}}}
\newcommand{\lemref}[1]{\tikzrefsize{\eqref{#1}}}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}
%======================================
\newtheorem{Th}{Theorem}[section]
\newtheorem{theorem}[Th]{Theorem}
\newtheorem{proposition}[Th]{Proposition} 
\newtheorem{lemma}[Th]{Lemma}
\newtheorem{corollary}[Th]{Corollary}
\newtheorem{definition}[Th]{Definition} 
\newtheorem{example}[Th]{Example}
\newtheorem{remark}[Th]{Remark}

%======================================
\newcommand{\rsnote}[1]{\marginpar{\scriptsize \bB \emph{RS:} #1 \e}}
\newcommand{\hwnote}[1]{\marginpar{\scriptsize \bR \emph{HW:} #1 \e}}

\newcommand{\zxw}[1]{\cite[#1]{poorCompletenessArbitraryFinite2023}}
\newcommand{\inftyfy}[1]{#1$\null_{\infty}$}
